Bounds on the conditional and average treatment effect with unobserved confounding factors

For observational studies, we study the sensitivity of causal inference when treatment assignments may depend on unobserved confounders. We develop a loss minimization approach for estimating bounds on the conditional average treatment effect (CATE) when unobserved confounders have a bounded effect on the odds ratio of treatment selection. Our approach is scalable and allows flexible use of model classes in estimation, including nonparametric and black-box machine learning methods. Based on these bounds for the CATE, we propose a sensitivity analysis for the average treatment effect (ATE). Our semi-parametric estimator extends/bounds the augmented inverse propensity weighted (AIPW) estimator for the ATE under bounded unobserved confounding. By constructing a Neyman orthogonal score, our estimator of the bound for the ATE is a regular root-$n$ estimator so long as the nuisance parameters are estimated at the $o_p(n^{-1/4})$ rate. We complement our methodology with optimality results showing that our proposed bounds are tight in certain cases. We demonstrate our method on simulated and real data examples, and show accurate coverage of our confidence intervals in practical finite sample regimes with rich covariate information.

==> acknowledgments.tex <==
\subsection*{Acknowledgements}

We would like to acknowledge useful comments, discussions, and
feedback with Stefan Wager and Nigam Shah on this work. SY would also like
to thank Mike Baiocchi for his discussions and encouragement to study
unobserved confounding.

SY was partially supported by a Stanford Graduate Fellowship, and HN was
partially supported by Samsung Fellowship. JCD was partially
supported by NSF CAREER Award CCF-1553086 and
the Office of Naval Research Young Investigator Award N00014-19-1-2288.
Research reported in this
publication was supported by the National Heart, Lung, and Blood
Institute; the National Institute Of Diabetes And Digestive And Kidney
Diseases; and the National Institute On Minority Health And Health
Disparities of the National Institutes of Health under Award Numbers
R01HL144555, R01DK116852, R21MD012867, DP2MD010478, and U54MD010724. The
content is solely the responsibility of the authors and does not
necessarily represent the official views of the National Institutes of
Health.


==> nu-estimation.tex <==
Let $\popprob(\covariate) = 1 + (\Gamma - 1)\P(Y(1) \ge \popfunc(x) | X =
x, Z=1)$. To estimate it, we propose to employ the sieve estimation method again.  Define the loss function
$\bar{\loss}: [1, \Gamma]^{\covspace} \times \R^{\covspace} \times (\covspace, \R)
\to \R$
\begin{equation*}
  \bar{\loss}(\probfunc; \funcparam, (\covariate, \outcome)) \defeq \half \left(
    1 + (\Gamma - 1)\indic{\outcome \ge \funcparam(\covariate)} -
    \probfunc(\covariate)  \right)^2,
\end{equation*}
and consider the minimization problem
\begin{equation}
  \label{eqn:opt-prob}
  \minimize_{\probfunc(\cdot)}
    ~ \treatedE[  \bar{\loss}(\probfunc; \popfunc, (\covariaterv, Y(1)))]
\end{equation}
over measurable functions.
Since $\popprob$ is the unique minimizer of the problem~\eqref{eqn:opt-prob},
the ideal sieve estimator for $\popprob$ minimizes the empirical version of \eqref{eqn:opt-prob}. However, this
requires knowledge of $\popfunc$, which itself needs to be estimated. Therefore, consider the following (nested) cross-fitting approach. Partition the samples in $\mathcal{I}_{-j}$ into two \emph{independent} sets,
and let $\what{\theta}_{1j}^{\nu_1}$ be an estimator of $\popfunc$ trained on the first
subset. For some sequence of sieve parameter spaces
\begin{equation*}
  \probspace_1 \subseteq  \cdots \subseteq \probspace_{n} \subseteq
  \cdots \subseteq \probspace,
\end{equation*}
estimate $\what{\nu}_{1,j}(x)$ by finding an (approximate) minimizer of the
following sieve approximation for the plug-in version of the population
problem~\eqref{eqn:opt-prob}
\begin{equation}
  \label{eqn:opt-emp-prob}
  \minimize_{ \probfunc(\cdot) \in 1 + (\Gamma -1)\probspace_{n}}
  ~\mathbb{E}_{n_{j2}}[  \bar{\loss}(\probfunc; \empfuncp, (\covariaterv, Y(1)))],
\end{equation}
where the expectation is with respect to the empirical distribution of the observations in the second set of $\mathcal{I}_{-j}.$ \noindent Section~\ref{sec:sieve-method} provides examples of reasonable choices of sieves that may be used.

\subsubsection[Convergence guarantees for nu1(x)]{Convergence guarantees for $\what{\nu}_1(x)$}
In this section, we provide convergence guarantees for the estimator in
Section~\ref{sec:semiparametric-method} for completeness. In order for the empirical plug-in for the
problem~\eqref{eqn:opt-emp-prob} to converge, the map
$x \mapsto P(Y(1) \ge \funcparam(x) | \covariaterv = \covariate, \treatmentrv=1)$ must be smooth for smooth functions
$\funcparam$ around $\popfunc$.
\begin{assumption}
  \label{assumption:prob-smooth}
  There exists $\probsmooth, \probradius > 0$, and a set
  $S \subset \holderball{\holdersmooth}{\holderradius}$ with
  $\popfunc \in S$
  such that
  \begin{enumerate}
  \item $P(\empfunc \in S|\treatmentrv=1) \to 1$ as $n \to \infty$
  \item for all $\funcparam \in S$,
    $x \mapsto P(Y(1) \ge \funcparam(x) | \covariaterv = \covariate, \treatmentrv=1)$
    belongs in
    $ \probspace \defeq \holderball{\probsmooth}{\probradius} \cap \left\{
      \probfunc: \covspace \to [0, 1] \right\}$.
  \end{enumerate}
\end{assumption}
\noindent For example, since $\ltwotp{\empfunc - \popfunc} = o_p(1)$, $S$ can
be a $\ltwotp{\cdot}$-neighborhood of
$\popfunc \in \holderball{\holdersmooth}{\holderradius}$, where $\treatedP(\cdot) = P(\cdot|Z=1)$, so long as the second
condition holds.

Since $\hat{\nu}(x)$ solves an empirical version of
problem~\eqref{eqn:opt-emp-prob} that uses the estimate $\empfuncp$ instead
of the true parameter $\funcparam$, it estimates the map
\begin{equation}
\label{eq:empirical-nu-map}
x \mapsto P(Y(1) \ge \popfunc(x) | \covariaterv = \covariate, \treatmentrv=1)
\end{equation}
insofar as \eqref{eq:empirical-nu-map} is smooth around $\popfunc$. Requiring that
$Y(1) | \covariaterv, \treatmentrv = 1$ has a Lipschitz cumulative
distribution guarantees this.
\begin{assumption}
  \label{assumption:lip-cdf}
  There exists $L_{\probfunc} > 0$ such that
  $t \mapsto \treatedP(Y(1) \ge t | \covariaterv)$ is
  $L_{\probfunc}$-Lipschitz almost surely.
\end{assumption}
\noindent For example, the above assumption holds if
$P_{Y(1) | \covariaterv, \treatmentrv = 1}(\cdot|X)$ has a bounded density with
respect to the Lebesgue measure for almost ever $\covariaterv$.

The following standard non-parametric rates
for estimating $\popprob$ are a consequence of using the finite dimensional
linear sieves examples given in Section~\ref{sec:sieve-method} with the plug-in empirical minimization problem \eqref{eqn:opt-emp-prob}. We defer its proof to
Appendix~\ref{section:proof-of-prob-sieve}.
\begin{restatable}{prop}{propprobsieve}
  \label{prop:prob-sieve}
  For $\covspace = [0, 1]^d$, let $\probspace_n$ be given by finite
  dimensional linear sieves considered in
  Examples~\ref{example:polynomials} or \ref{example:splines}
  with
  $\comp_n \asymp n^{\frac{1}{2\holdersmooth + \covdim}} (\log n)^{-\frac{4}{2\holdersmooth + \covdim}}$.
  % $\comp_n \approx n^{\frac{1}{2 \probsmooth + \covdim}}$
  Let
  Assumptions~\ref{assumption:lebesgue-equiv},~\ref{assumption:prob-smooth},~\ref{assumption:lip-cdf}
  hold, and let $\empprob$ be an approximate empirical minimizer to the
  problem~\eqref{eqn:opt-emp-prob} satisfying
    \begin{equation*}
    \emptreatedE[  \bar{\loss}(\empprob; \empfuncp, (\covariaterv, Y(1)))]
    \le   \inf_{ \probfunc \in 1 + (\Gamma-1)\probspace_n}
    \emptreatedE[ \bar{\loss}(\probfunc; \empfuncp, (\covariaterv, Y(1)))]
    + O_p\left( \left(\frac{(\log n)^4}{n} \right)^{\frac{2\holdersmooth}{2\holdersmooth + \covdim}} \right).
  \end{equation*}
  Then,
  $\norm{\empprob - \popprob}_{2, \treatedP} = O_p\left(
    n^{-\frac{\holdersmooth}{2\holdersmooth + \covdim}} + \ltwotp{\empfuncp -
      \popfunc} \right)$.
\end{restatable}
\noindent For example, consider a procedure that partitions the sample into
two sets, and uses the first subset to estimate $\empfunc$ as in
Theorem~\ref{thm:sieve}. Using the other subset to compute $\empprob$,
Proposition~\ref{prop:prob-sieve} and Theorem~\ref{thm:sieve} yield
$\norm{\empprob - \popprob}_{2, \treatedP} = O_p\left(
  n^{-\frac{\holdersmooth}{2\holdersmooth + \covdim}} \right)$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

